Colored Transparent Object Matting from a Single Image Using Deep Learning

This paper proposes a deep learning based method for colored transparent object matting from a single image. Existing approaches for transparent object matting often require multiple images and long processing times, which greatly hinder their applications on real-world transparent objects. The recently proposed TOM-Net can produce a matte for a colorless transparent object from a single image in a single fast feed-forward pass. In this paper, we extend TOM-Net to handle colored transparent object by modeling the intrinsic color of a transparent object with a color filter. We formulate the problem of colored transparent object matting as simultaneously estimating an object mask, a color filter, and a refractive flow field from a single image, and present a deep learning framework for learning this task. We create a large-scale synthetic dataset for training our network. We also capture a real dataset for evaluation. Experiments on both synthetic and real datasets show promising results, which demonstrate the effectiveness of our method.

==> realresult/lenscol/Log <==
Input_root: D:\URFP\realcoloredresult\lastchance\collens
dir_list: D:\URFP\realcoloredresult\lastchance\collens\dir_list.txt
PSNR_bck: 11.561163SSIM_bck: 0.731631
PSNR: 17.464506SSIM: 0.807933

